A unified graphical approach to random coding for multi-terminal networks

A unified approach to the derivation of rate regions for single-hop memoryless networks is presented. A general transmission scheme for any memoryless, single-hop, k-user channel with or without common information, is defined through two steps. The first step is user virtualization: each user is divided into multiple virtual sub-users according to a chosen rate-splitting strategy which preserves the rates of the original messages. This results in an enhanced channel with a possibly larger number of users for which more coding possibilities are available. Moreover, user virtualization provides a simple mechanism to encode common messages to any subset of users. Following user virtualization, the message of each user in the enhanced model is coded using a chosen combination of coded time-sharing, superposition coding and joint binning. A graph is used to represent the chosen coding strategies: nodes in the graph represent codewords while edges represent coding operations. This graph is used to construct a graphical Markov model which illustrates the statistical dependency among codewords that can be introduced by the superposition coding or joint binning. Using this statistical representation of the overall codebook distribution, the error probability of the code is shown to vanish via a unified analysis. The rate bounds that define the achievable rate region are obtained by linking the error analysis to the properties of the graphical Markov model. This proposed framework makes it possible to numerically obtain an achievable rate region by specifying a user virtualization strategy and describing a set of coding operations. The largest achievable rate region can be obtained by considering all the possible rate-splitting strategies and taking the union over all the possible ways to superimpose or bin codewords.

==> ChannelModel.tex <==


\section{Channel Model}
\label{sec:Channel Model}



\begin{figure}
\centering
%\vspace{- 1.8 cm}
\includegraphics[width=.48 \textwidth]{GPchannel}
\vspace{-3.6 cm}
\caption{The Gelfand-Pinsker channel.
}
\vspace{-0.8 cm}
\label{fig:GPchannel}
\end{figure}


In the Gelfand-Pinsker (GP) channel, also depicted in Fig. \ref{fig:GPchannel}, the output $Y^N$ of a point to point channel is obtained as a random function of the input $X^N$ and a state sequence $S^N$ which is known at the transmitter but not at the receiver.
%
%The state sequence is known at the transmitter but not at the receiver, thus modelling the scenario in which the transmitter has knowledge of the interference affecting the comminution channel but the receiver has not.
%
In this model, the transmitter wishes to communicate the message $W \in \{1 \ldots 2^{NR} \}$ through the channel input $X^N$ to its intended receiver.
%
This receiver has access to the channel the output sequence $Y^N$ and uses it to produce an estimate $\Wt$ of the transmitted message $W$.
%
The output $Y^N$ is obtained from the input $X^N$ and a state sequence $S^N$ and through $N$ successive uses of the  memoryless channel $P_{Y|X,S}$, that is
\ea{
Y^N  \sim  P_{Y|X,S}^N(X^N,S^N)
\label{eq: GP channel}
}
%
The encoder has non-causal access to the state sequence $S^N$, obtained from iid draws from the distribution $P_S$, and can thus design the channel input $X^N$ has to minimize its adverse effects on the channel output $Y^N$.
%
%For this channel, the goal is to design an encoder and a decoder such that $w$ can be successfully recover from the channel out.
%%
%To rigorously define this goal, we introduce the concept of code, achievable rate and capacity.
%

To study this channel model,  standard definitions of  code, achievable rate and capacity are employed.



\begin{definition}{\bf Code. }
A $(2^{N R}; N)$ code for the  GP channel  consists of the message set $\Wcal=[1 \ldots 2^{N R}]$, an encoding
functions and a decoding functions, respectively defined as:
%The encoding function at transmitter  is defined as
\pp{
X^N &: \Wcal  \times \Scal^N \goes \Xcal^N,  \quad &X^N = X^N(W, S^N), \\
\Wh &: \Ycal^N \goes \Wcal,   &\Wh = \Wh(Y^N) \\
}
where $\Qcal^N$ is the support of the random variable (RV) $Q^N$.
%
%Similarly, the decoding function at the receiver is defined as
%\ean{
%\widehat{W} & : \Ycal \goes \Wcal \\
%}
\end{definition}

The rate $R$ is achievable if there exists a sequence of codes such that we have
that the probability of a decoding error goes to zero as the block length $N$ goes to infinity.

\begin{definition}{\bf Achievable Rate.}
Let the the probability of decoding error for a code $(2^{N R}; N)$ be defined as
\ea{
P_e(2^{N R}; N)=\Pr \lsb  \Wh (Y^N)\neq W \rsb,
}
then, a rate $R\in \Rbb^+$ is said to be  achievable if there exists a sequence of codes such that
\ea{
\lim_{N \goes\infty}  P_e(2^{N R};N)  = 0
\label{eq:def error probability}
}
Note that the error probability in \eqref{eq:def error probability} is averaged over all state sequences and messages.
%
%The capacity $C$ is the supremum of all the achievable rates.
\end{definition}


\begin{definition}{\bf Capacity and  Approximate Capacity.}
%The rate $R$ is achievable if there exists a sequence of codes such that, for $W$ uniformly distributed over $W_N$, we have
%\ea{
%\lim_{N \goes\infty}  P_e^N = \lim_{N \sgoes \infty} \Pr \lcb \bigcup_{j=1}^M  g_{j,N}(Y_j^N)\neq W \rcb  =0.
%\label{eq:def error probability}
%}
%Note that the error probability in \eqref{eq:def error probability} is averaged over all state sequences and messages.
%
The capacity $C$ is the supremum of all the achievable rates.
%
The region $R^{\rm IN}$ is said to be an inner bound to the capacity region if $R^{\rm IN} \leq C$.
Similarly, the region $R^{\rm OUT}$ is an outer bound to capacity if $R^{\rm OUT} \geq C$.
%
Inner and outer bounds for which
\ea{
R^{\rm OUT}-R^{\rm IN} \leq \Delta
}
for some constant $\Delta \in \Rbb^+$ are said to characterize the capacity to within an additive gap of $\Delta$ bits-per-channel-use (bpcu).
%
%Similarly, an inner bound and outer bound for which
%\ea{
%\f {R^{\rm OUT}}{R^{\rm IN}} \leq \Delta
%}
%for some constant $\Delta \in \Rbb^+$ are said to characterize the capacity to within a \underline{multiplicative gap} of $\Delta$.
%
\end{definition}


%
%%
%%
%    %\subsection{Dirty Paper Channel with Fast Fading Dirt  with No Receiver Channel Side Information (DPC-FFD-NCSI)}
%
The ``writing dirty paper '' (WDP) channel was introduced in \cite{costa1983writing} and is the version of the GP channel in which the input is subject to a second moment constraint and the output is obtained as a linear combination  of the channel input, the state sequence and a Gaussian iid noise sequence, i.e.
\ea{
Y^N = X^N+S^N+Z^N
\label{eq:Dirty Paper Channel}
}
for $\Ebb \lsb |X_i|^2 \rsb  \leq P$ and  $Z_i \sim \Ncal(0,1),  \ iid$ for  $i \in [1\ldots N]$.

%%both the noise and the state
%
\medskip
%
%\begin{description}
%  \item[] 
%  \item[] 
%  \item[] 
%\end{description}
%We next introduce  three special cases of the GP channel which will be relevant in the following:
%
%In the literatere, the most studied
%
In the following we shall study  a variation of the channel in \eqref{eq:Dirty Paper Channel} in which the state sequence $S^N$ is multiplied by a fast fading sequence $A^N$.
%
We consider both the case in which $A^N$ in unknown at both the transmitter and the receiver and the case in which $A^N$ is known only an the receiver.
%
Both these models are a special case of the GP channel  in Fig. \ref{fig:GPchannel}.


\medskip
\noindent
$\bullet$
% {\bf Dirty Paper Channel with Fast Fading Dirt and No Channel Side Information (DPC-FFD-NCSI)}
{\bf Writing on Fast Faded Dirt with No Channel Side Information (WFFD-NCSI) channel}, also depicted in Fig. \ref{fig:WritingOnFadingDirtNCSI},
is the DPC in which the state sequence is multiplied by a fast fading sequence $A^N$ obtained through iid draws from the distribution $P_A$, i.e.
\ea{
Y^N = X^N+A^N S^N+Z^N.
\label{eq:Dirty Paper Channel NCSI}
}
The sequence $A^N$ is not known at either the transmitter or the receiver.


\medskip
\noindent
$\bullet$ { \bf Writing on Fast Faded Dirt with Receiver Channel Side Information (WFFD-RCSI) channel}, also depicted in Fig. \ref{fig:WritingOnFadingDirtRCSI},  is obtained from the WFFD-NCSI by providing the receiver with the fast fading sequence. This can be model as $A^N$ be an additional channel output, that is
\ea{
Y^N = \lcb  \p{
X^N+A^N S^N+Z^N \\
A^N
}
\rnone
\label{eq:Dirty Paper Channel RCSI}
}
%
%
%In the following we focus mostly on the  DPC-FFD-NCSI and the DPC-FFD-RCSI, while the DPC is presented mostly for clarity and completeness.
%%\subsection{Dirty Paper Channel with Fast Fading Dirt  with No Receiver Channel Side Information (DPC-FFD-NCSI)}
When we intend to refer to both the WFFD-NCSI and the WFFD-RCSI, we will simply refer the two models as WFFD    .
%
%\begin{figure}
%\centering
%%\vspace{- 1.8 cm}
%\includegraphics[width=.6 \textwidth]{WritingOnDirtPaper}
%\vspace{-3.3 cm}
%\caption{The Dirty Paper Channel (DPC).
%The dotted line represents the state information provided at the transmitter.
%}
%\vspace{-.5 cm}
%\label{fig:WritingOnDirtPaper}
%\end{figure}
%

%
%\begin{figure}
%\centering
%%\vspace{- 1.8 cm}
%\includegraphics[width=.5 \textwidth]{WritingOnFadingDirtV1}
%\vspace{-3.8 cm}
%\caption{The Dirty Paper Channel with Fast  Fading Dirty (DPC-FFD).
%}
%\vspace{-.5 cm}
%\label{fig:WritingOnFadingDirtNCSI}
%\end{figure}
%
%
%\begin{figure}
%\centering
%%\vspace{- 1.8 cm}
%\includegraphics[width=.5 \textwidth]{WritingOnFadingDirtRCSIV1}
%\vspace{-3.8 cm}
%%\vspace{-1.5 cm}
%\caption{The Dirty Paper Channel with Fast Fading Dirty and Receiver Channel Side Information (DPC-FFD-RCSI).
%%
%}
%\vspace{-.5 cm}
%\label{fig:WritingOnFadingDirtRCSI}
%\end{figure}


\begin{figure}[ht]
\centering
\subfigure[WFFD with No Channel Side Information  (WFFD-NCSI).]{
   \includegraphics[width =.48 \textwidth] {WritingOnFadingDirtV1}
   %\vspace{-3.8 cm}
   \label{fig:WritingOnFadingDirtNCSI}
 }
 \subfigure[WFFD with Receiver Channel Side Information  (WFFD-RCSI).]{
   \includegraphics[width =.48 \textwidth] {WritingOnFadingDirtRCSIV1}
   %\vspace{-3.8 cm}
   \label{fig:WritingOnFadingDirtRCSI}
 }
\caption{Writing on Fast Faded Dirt (WFFD) channel.}
\label{fig:MAC schemes}
\end{figure}
\bigskip

%
%Regarding the DPC-FFD-NCSI and DPC-FFD-RCSI we can observe the interplay between state and fading.
%
In general, the sequence $S^N$ or $A^N$ can have any mean but we shall restrict ourselves to the case in which $S$ has mean zero.

\begin{rem}{\bf On the mean of the state and fading distribution.}
\label{rem:On the mean of the state and the fading distribution}
The channel output in \eqref{eq:Dirty Paper Channel NCSI} can be rewritten (by dropping the superscript $N$) as:
% follows (by dropping the index $i$)
\ea{
Y
& =X+c \lb  A_0- \mu_A \rb \lb S_0-\mu_S \rb +Z \nonumber \\
%
& =X + c \lb A_0 S_0 - \mu_A S_0- \mu_S  A_0+ \mu_A \mu_S  \rb +Z,
\label{eq:expression means}
}
where $\Ebb[A]=\mu_A$, $\Ebb[S]=\mu_S$,  $A_0= A-\mu_A$ and $S_0= S-\mu_S$.
%have the same distribution as $A,S$ but are shifted in the origin.
%
%We can now consider each term separately and draw some intuition on the composition of the output.
%Consequently the channel output can be seen the summation of the following terms:

Each of the term in \eqref{eq:expression means} can be seen as follows:

%
%For these reasons, we can focus only on fading distributions that have $\mu_A=0$.

\noindent
$\bullet$  the term $c \mu_A S_0$ can be pre-cancelled with Costa coding by the transmitter as in \cite{costa1983writing} (Costa pre-coding in the following).

\noindent
$\bullet$ the term $c \mu_S  A_0 $ can be subtracted from the output in the WFFD-RCSI.  In the WFFD-NCSI is unknown at both the receiver and the transmitter  and is thus equivalent to additive noise. For these two reasons, we can restrict ourselves to the case in which $\mu_S=0$
%
%Without receiver fading knowledge,

\noindent
$\bullet$ $c A_0 S_0$  requires the cooperation of  both transmitter and receiver, since they each have a knowledge of one of the terms in the multiplication.
%can only be jointly managed by both transmitter and receiver, since they each have a knowledge of one of the terms of the multiplication.
%
%Note that scaling by $k_A k_S $ is used to express the fact that we can re-scale either the fading or the state without affecting the capacity of the channel.
%%
%For the reason above we focus on the scenario in which  the variance of $A$ and $S$ is normalized one.
\end{rem}


%
%%
%%\subsection{}
%%\label{sec:Generalized channel}
%\blue{merge to remarks\\
%%
%Also just set the mean to zero: it's just making things a mess!
%}

Additionally, the RVs $S$ or $A$ can have any variance, but it is sufficient to consider to the case in which they both have unitary variance.


\begin{rem}{\bf On the variance  of the state and fading distribution. }
\label{rem:variance  of the state and fading}
The channel output in \eqref{eq:Dirty Paper Channel NCSI} can be rewritten (by dropping the superscript $N$) as:
\ea{
Y & =X+c \sigma_A \sigma_S \f {A}{\sigma_A} \f {S} {\sigma_S} +Z
\label{eq:variance  of the state and fading}
}
where $\sigma_A=\var[A]$ and $\sigma_S=\var[S]$.
%
The expression in \eqref{eq:variance  of the state and fading} implies that the capacity of the channel is a
function only of the value $c$ and the power constraint $P$ while the variance of $S$ and $A$ can be set to one without loss of generality.
%
%
%Consider a more general channel than that of \eqref{eq:Dirty Paper Channel NCSI} in which %is which the state is Gaussian with any mean and variance
%% and the fading and the noise are not restricted to have unitary variance.
%%%,the fading is not restricted to have unitary variance and the noise has any variance,
%%that is
%\ea{
%\Yt &= X + \ct \At \St + Z
%\label{eq:generalized channel model}
%}
%for
%\eas{
%%& \St_i    \sim \Ncal(\mu_{\St},\sgs_{\St}),  \quad \Zt_i \sim \Ncal(0,\sgs_Z), \\
%& \St \ \ST \ \Ebb[\St] = \mu_S, \quad \var[\At] = \sgs_S \\
%& \At \ \ST \ \Ebb[\At] = \mu_A, \quad \var[\At] = \sgs_A,
%}
%%and $\Yt_i=\Xt_i+\ct \At_i \St_i+\Zt_i$,
%%\ea{
%%\Yt_i=\Xt_i+\ct \At_i \St_i+\Zt_i.
%%\label{eq:generalized channel model}
%%}
%for some $\ct \in \Rbb$ and where $\Xt$ is subject to the average power constraint $\Ebb[|\Xt|^2]\leq \Pt$.
%%
%The model in \eqref{eq:generalized channel model} is shown to be identical to the model in \eqref{eq:Dirty Paper Channel NCSI} by considering the equivalent channel output
%\ea{
%Y=\f {\Yt_i} {\sigma_Z}=\f {\Xt_i}{\sigma_Z}+\ct \f{\sigma_A \sigma_S} {\sigma_Z} \lb \f{\At_i} {\sigma_A} \f{\St_i}{\sigma_S} \rb +\f{\Zt_i}{{\sigma_Z}}.
%\label{eq:equivalence models}
%}
%which has the same distribution as the channel output in \eqref{eq:Dirty Paper Channel NCSI} for
%\ea{
%%& c = \ct \f{\sigma_A \sigma_S} {\sigma_Z},  \quad  S = \St_i / \sigma_S   \quad & A = \At_i / \sigma_A  \nonumber\\
% c &= \ct \sigma_A \sigma_S / \sigma_Z,  \quad  S = \St_i / \sigma_S   \quad  A = \At_i / \sigma_A  \nonumber\\
% X &= \Xt_i / \sigma_Z , \quad \quad  \ \ P=\Pt / \sigma_Z
%\label{eq:equivalence channel}
%}
\end{rem}

%The equivalence in \eqref{eq:equivalence models} implies that we can re-scale the fading or the state without affecting the capacity of the channel, as long as the equivalence in \eqref{eq:equivalence channel} is preserved.
Rem.  \ref{rem:variance  of the state and fading} implies that we can re-scale the fading or the state without affecting the capacity of the channel,
as long as the product of the variances is kept constant.
%
This means that one cannot properly distinguish the magnitude of the fading with respect to the magnitude of the state since even a small amount of fading can be amplified by a large state variance and viceversa.
%, thus making impossible for the encoder to pre-code against its effect.
%
%
%%
%In Dirty Paper Channel with Fast Fading Dirt (DPC-FFD), also depicted in Fig. \ref{fig:WritingOnFadingDirt}, the channel output is obtained as
%\ea{
%Y^N = X^N + c A^N S^N + Z^N,  \quad c\in \Rbb
%\label{eq:Dirty Paper Channel NCSI}
%}
%and where $X^N$ is the channel input, $S^N$ the state sequence,  $A^N$ the ergodic fading realization and $Z^N$ the additive noise.
%%
%The channel input $X^N$ is subject to a second moment constraint $\Ebb \lsb |X_i|^2 \rsb  \leq P, \ i \in [1 \ldots N]$ while the state $S^N$ and the noise term $Z^N$ are distributed as
%\ea{
%S_i \sim \Ncal(\mu_S,1), \quad Z_i \sim \Ncal(0,1),  \quad i.i.d. \ i \in [1\ldots N]
%}
%where $\Ncal(\mu,\sgs)$  indicates the Gaussian Random Variable (RV) with mean $\mu$ and variance $\sgs$.
%%
%The fading sequence $A^N$ is obtained with $N$ iid draws from a distribution $P_A$ with variance one and mean $\mu_A$.
%%
%The state sequence $S^N$ is assumed to be non-causally available at the transmitter while fading sequence $A^N$ is unknown at both the transmitter or the receiver.
%
%
%\subsection{Dirty Paper Channel with Fast Fading Dirt  with Receiver Channel Side Information (DPC-FFD-RCSI)}
%
%A model related  to the DPC-FFD in Fig. \ref{fig:WritingOnFadingDirt} is the model in which the fading sequence $A^N$ is provided to the receiver.
%%
%We refer to this model as the Dirty Paper Channel with Fast Fading Dirty and Receiver Channel Side Information (DPC-FFD-RCSI), also depicted in Fig. \ref{fig:WritingOnFadingDirtRCSI}.
%%
%For the DPC-FFD-RCSI the receiver side information,$A^N$, can be seen as an additional channel output, that is,
%the channel  output is the vector $Y'^N=[Y^N \ A^N]$ instead of only the vector $Y^N$ in \eqref{eq:WritingOnFadingDirtChannelModelGeneral}.
%
%
%\subsection{Dirty Paper Channel with with Phase Fading and Receiver Channel Side Information (DPC-FFD-RCSI)}
%
%
%
%In the following we deal with general distributions of $S$ and $A$ but state some of the results for specific distributions.
%
%On such restrition is on the entropy of a variable with unitary variance: given the ``Gaussian Maximizes Entropy'' (GME) property we have that
%\ea{
%H(V)=\f 12 \log (\al),  \quad \al \in [0,1]
%\label{eq:bound H is al}
%}
%for some RV $V$ with unitary variance.
%
%
%Another restriction is on the average probability distribution for a variable, namely we define
%\ea{
%f_{\max}(V)= \max_{I} \f 1 I \int_I \diff P_V
%\label{eq:definition f max}
%}
%and where $I$ is a closed set in  $\Rbb$.
%
%That is $f_{\max}$ has the meaning of an average density of the distribution of $A$.
%
%A high value of $f_{\max}$ indicates that the  distribution is highly concentrated around some interval, while a small value of $f_{\max}$ indicates that the distribution is generally spread over it's support.
%

